Capstone: Mobility Modeling on Smartphones to Achieve Privacy by Design

Sharing location traces with context-aware service providers has privacy implications. Location-privacy preserving mechanisms, such as obfuscation, anonymization and cryptographic primitives, have been shown to have impractical utility/privacy tradeoff. Another solution for enhancing user privacy is to minimize data sharing by executing the tasks conventionally carried out at the service providers' end on the users' smartphones. Although the data volume shared with the untrusted entities is significantly reduced, executing computationally demanding server-side tasks on resource-constrained smartphones is often impracticable. To this end, we propose a novel perspective on lowering the computational complexity by treating spatiotemporal trajectories as space-time signals. Lowering the data dimensionality facilitates offloading the computational tasks onto the digital-signal processors and the usage of the non-blocking signal-processing pipelines. While focusing on the task of user mobility modeling, we achieve the following results in comparison to the state of the art techniques: (i) mobility models with precision and recall greater than 80%, (ii) reduction in computational complexity by a factor of 2.5, and (iii) reduction in power consumption by a factor of 0.5. Furthermore, our technique does not rely on users' behavioral parameters that usually result in privacy-leakage and conclusive bias in the existing techniques. Using three real-world mobility datasets, we demonstrate that our technique addresses these weaknesses while formulating accurate user mobility models.

==> abstract.tex <==
%!TEX root = main.tex
\begin{abstract}

Context-aware services are becoming increasingly dependent on user profiling and behavioral tracking.   
In the case of location-based services, sharing location traces with third party providers has privacy implications. 
A solution for enhancing user privacy is to minimize data sharing by executing the tasks, conventionally carried out at the service providers end on to the user’s smartphones. 
Thereby, significantly reducing the volume of data shared with the untrusted entities, relying on a proactive and de-facto privacy design. 
However, tasks such as user mobility modeling are computationally expensive, when to be performed on power and resource-constrained devices. 
In this context, we propose a new perspective on geospatial computation by treating trajectories as space-time signals. 
Processing signals rather than three dimensional trajectories is beneficial due to: (1) reduced dimensionality, (2) compressed data magnitudes, and (3) ability to exploit digital-signal processors to offload computation tasks.  
However, this brings up two key questions: Do the space-time signals retain all the key information contained in a trajectory? and, How accurate are the formulated mobility models? 
To this end, we present a technique for translating the trajectories into continuous signals and facilitate their interpretation by presenting the inter-domain mapping between the trajectory components and the signal elements.
A key contribution of this paper is a technique for constructing the user mobility model by only using the space-time signals. 
Using real world datasets, we show that our approach yields the following advantages: (1) accurate mobility models with precision and recall rates exceeding 80\%, (2) independence from an {\it{a–priori}} selection of behavioral parameters that involve high bias in the existing techniques, and the (3) reduction in complexity.   


Models of human mobility have broad applicability in fields such as mobile computing, urban planning, and ecology. 

Nodes in STEPS have preferential attachment
to favorite locations where they spend most of their time.

Human mobility is known to have a significant impact on performance of net-
works created by wireless portable devices e.g. MANET, DTN. Unfortunately,
there is no model that is able to capture all the characteristics of human mobility
due to its high complexity.


n this paper we introduce Spatio-TEmporal Para-
metric Stepping (STEPS) - a new powerful formal model for human mobility or
mobility inside social/interaction networks.

Understanding human mobility is of great importance to various applications, such as urban planning, traffic scheduling, and location prediction. 

Understanding human mobility has been widely recognized as a corner-stone task for various applications, ranging from urban planning and traffic scheduling to location prediction and personalized activity recommendation.


Human Mobility can be modelled as a Discrete-time Markov chain

Semantic locations modeled as states (𝒙𝒕)

Inter-state transitions governed by probabilities:




  

\end{abstract}



==> attack_surfaces.tex <==
\section{Attack Surfaces}
\label{sec:intro}

We also answer the following questions. 


knowing which stations aren't supervised and hence allow you to exit and buy a ticket for that one journey is a lot cheaper than being hit with a penalty fare from a grumpy railway worker. 

That said, inspections are fairly frequent. I often see people wait until inspectors get on board and then purchase or validate a ticket, or stand up and get off at the next stop (which will never be more than a block or two away). 

\begin{itemize}
	\item Which stops/transport lines are controlled at very high frequency?
	\item At what hours of the day is controlling prominent?
	\item Is there any correlation between the stop/line and the time it is controlled?
	\item At which stops is controlling performed outside the vehicle?
	\item Given the current controller location, is it possible to predict the next location?
	\item Are there any observable patterns in weekday/weekend/seasonal  
\end{itemize} 

%TODO: Somethings about the legitimacy of the data. 

\subsection{Selective ticket purchasing}

In order to carry out this akt, we first need to calculate the probabilities of getting controlled at all the stops and tag each one with the respective probability of getting caught.  
Therefore, we analyzed the data to estimate the control probability at each stop and at every line as shown in Figure Blah. 
We found a total of NS number of stops and NL number of lines being controlled. 
Out of the NS stops, only a x\% are controlled over a frequency of f every week. 
Overall, we find that only n number of stops controlled above a frequency of f in last five years. 
Furthermore, there exists a total of N number of lines consisting of 2 metro lines and n bus lines. 
Out of which the metro lines are controlled at a frequency of x every week and out of the N bus lines only n are controlled above a frequency of f. 
From the above stats, it is clear as to effectively avoid purchasing the tickets by estimating the risk associated with getting controlled at the respective stops. 

A raise of morale could be one effect. However, people will buy tickets for lines where inspections are foreseen but the contrary may happen elsewhere. Not all inspections should be revealed; instead, it could be an option to publish controls and results afterwards.

To take this one step ahead, we correlated the controls at the stops and lines with the temporal aspect and found strong correlations. 
We depict the results in Figure Blah. 
As seen, certain stops are only controlled at specific time instances. 
Given this knowledge, it is fairly trivial to either avoid those stops and lines completely or only purchase tickets when traveling through these stops at only certain times. 


\subsection{Avoiding high risk stops}

Another insight discovered from the data shows that the controls can be placed at the stops either inside the lines or outside the stops when the passengers exists the vehicle. 
Therefore, we analyzed the stops where the controls are performed outside or inside the vehicle and discovered strong correlations between the position of controlling and stops. 
As seen in Figure Blah, the stops having the probability of control over x\% also has the probability of getting controlled outside the vehicle. 
Therefore, it is possible to avoid to such stops if a passenger does not posses a valid ticket and get down at either the previous or the next stop.   


\subsection{Re-routing attack}

We also analyzed the predictability of movement between the stops with respect to the current position and time. 
In figure blah, we show the confidence of movement between the stops controlled at high frequency. 
As seen, some of the stops have confidence higher then 70\%, this information can be used to predict where the controllers will go next given their current position. 
Similarly, we estimated the prediction over all the stops using the last five years of data and achieve an average of 73\% accuracy in predicting the next location. 
This information can be used to carry our rerouting atks wherein a traveller can change the route between the origin and destination, significantly lowering the probability of getting controlled. 
As shown in the figure below, some of the reroutes by skipping the main hubs even achieve lower travel times compared to routes often followed by the passengers. 
This is off course provide the time synchronization is managed optimally. 


\subsection{Exploiting seasonality patterns} 

The data analysis also revealed some patterns between weekday and weekend and various seasons. 
For example we discovered that the controlling frequency becomes almost 30\% lower on weekdays and in the last quarter of the year. 
Additionally the controls performed during these times are only restricted to 4-5 hubs in the city which are easily avoidable by following alternate routes. 
Therefore a traveler can avoid purchasing tickets during such times without significantly increasing the probability of getting controlled.  





==> conclusion.tex <==
%!TEX root = main.tex



\section{Conclusion}\label{sec:conclusion}

With the growing ubiquity of location-aware mobile devices, the ability to analyse and predict mobility on a large scale is becoming possible, opening new opportunities but also posing new challenges.
Furthermore, with mobile devices becoming more powerful every day, it becomes possible to compute mobility predictions locally, i.e., without resorting to backend servers.
Yet traditional approaches to mobility prediction rely on processing large datasets on powerful backend servers.
This makes mobility prediction quite tedious and slow.
In addition, such centralized approaches come with a major location privacy concern, threatening the success of widespread adoption of LBS in the coming days. 
This enforces a real need to restrict computations involving sensitive user data on a local mobile device. 

To address these issues, we introduce \mobidict, a realtime mobility prediction system, to provide swift 
next place predictions. Our approach couples the prediction system with dynamic user mobility behaviours
to restrict the data required for model training to short durations as opposed to conventional training
approaches. This achieves accuracies exceeding 50\% for about 40\% of the users contained in the 
dataset for 2-MMC and RRN predictors. We also examine periods where our system accuracy, even exceeds
the baselines. Thus exhibiting that large amount of training data is not an absolute requirement to 
produce viable next place predictions. We also evaluate the computational cost associated with our approach 
and theoretically validate the feasibility to operate on a mobile device. 

We observe that certain family of predictors are more suited for particular mobility behaviours. Our 
future work will be an attempt to have an ensemble approach in the system to select a suitable predictor
in realtime according to behavioural changes, to attain higher accuracies. We will also focus to 
quantify the computational cost of the approach on an actual mobile device to confirm our hypothesis. Another
area will be to optimise the process so as to have fewer number of model updates that will intern contribute
to the cost.\newline

\textbf{Acknowledgment.} 
This work is partially supported by the Swiss National Science Foundation grant 146714 and 157160.


==> data_source.tex <==
\section{Data Source}
\label{sec:data_source}

In order to estimate the attack surfaces possible for avoiding the public transport controls, we analyze the crowd-sourced data containing the locations and timestamps of the ticket controls. 
%TODO: Figure out the right word for crowd-sourcing data - participatory sensing ? or citizen science data ?
Several activists who are protesting against expensive subscriptions for using the public transport in a city and others who wish to make public transport free have formulated several platforms.
Such platforms provide the users (general public from the respective city) means to update the locations where the controlling is taking place and as well to view this information. 
Several of such platforms exist in Europe where the data can be accessed depending on the user's city. 
Farebandit{\footnote{Farebandit:farebandit.net}} is one of such services which regularly updates the current locations being controlled using crowd-sourced data in cities such as Berlin, Paris, Stockholm, Vienna and others.
This data is collected via mobile applications {\footnote{Busted App: busted-app.com}}{\footnote{Fare2Bandit: play.google.com/store/apps/details?id=revizorwatch.cz}} which allow users to update the control locations. 
Furthermore, there are also twitter accounts that update the current controller positions{\footnote{Biljettkontroller: twitter.com/biljettinfo}}{\footnote{Busted-App Lausanne: twitter.com/BustedLAUSANNE}} by using the data streaming from the application. 

In this paper, we retrieve this data from one city in Switzerland as it tops all the other countries in losses related to fore-dodging. 
This data is (retrieved) from the twitter account linked to the application BustedLAUSANNE[cite]. 
The twitter account pulls the latest update made via the application and formats it in to a tweet. 
Over a period of five years from 2013 to 2017, we retrieve more than thirteen thousand tweets containing the timestamps and locations of the control checks. 
Our analysis reveals an average of five tweets per day (weekdays) and two tweets on weekends. 
The city under consideration, {\bf{Lausanne}} is relatively small with an area of 41.37~$km^2$ and a population density of 133,897 habitants according to the 2015 census report~\cite{lausanne}.
The application has a user base of more than 20,000~\cite{gogle_play}. 
With over five international universities, Lausanne is primarily a student city which is a major user base of the said application. 
This demographics effects the data quality as the population using the application is spread across the city due to the university locations.  
Additionally, no timing constraints due to varying schedules of classes does not restrict the application usage to only certain times.
This essentially mitigates several biases associated with the data as the user base provides a coverage in space and time.   

   
However, other issues such as the data authenticity, uncertainty, accuracy and the legality aspects remain to be answered. 
Some key goals while working with crowd-sourced data are data quality, latency toleration levels, precision, coverage and diversity. 


\begin{table}[t!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cc}
\hline
\textbf{Criteria} & \textbf{Label} \\ \hline
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{333333} crowd interest} & {\color[HTML]{333333} interested} \\ 
crowd intention & well informed/malicious \\ 
\rowcolor[HTML]{C0C0C0} 
crowd ability & capable \\ 
tolerance for ambiguity & medium \\ 
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{333333} availability} & {\color[HTML]{333333} easily available} \\ 
sensitivity & sharable \\ \hline
\end{tabular}%
}
\caption{Micro-benchmarks of enclave tasks}
\label{tbl:bench_enc}
\end{table}


As this data is collected through human workers who often make mistakes, either due to the difficulty of the task at hand or due to inadequate expertise or diligence, we analyze where mistakes might happen and check the cost associated with the mistake. 
As the end users are the same as the workers who will eventually provide the data. 
In this case the cost associated with an error is high, however as human workers need to be compensated, the error rate is significantly lower. 
Another important factor is the latency in the crowdsourcing environment, however marking the place in an application with a preset menu of all the possible control points is fairly quick. 
Regarding the legality of the application, the act of informing others regarding the controller positions is legal and falls under the same jurisdiction as the popular navigation application {\bf{Waze}} which allows people to mark locations of police or speed traps as people have the right to communicate and to free speech.
It is similar to flashing headlights to warn others for speed traps.  
Although a problem here is regarding the fake location checkins by the police officers themselves as seen in Miani [] where the maze application  was used to flood the database with false locations for police speed traps. 
Such problems are resolved by involving a large number of participants where voting or triangulation based schemes can be used to remove and detect any irregularities and to increase the confidence in the data.  


